Consistent Range Approximation for Fair Predictive Modeling

This paper proposes a novel framework for certifying the fairness of predictive models trained on biased data. It draws from query answering for incomplete and inconsistent databases to formulate the problem of consistent range approximation (CRA) of fairness queries for a predictive model on a target population. The framework employs background knowledge of the data collection process and biased data, working with or without limited statistics about the target population, to compute a range of answers for fairness queries. Using CRA, the framework builds predictive models that are certifiably fair on the target population, regardless of the availability of external data during training. The framework's efficacy is demonstrated through evaluations on real data, showing substantial improvement over existing state-of-the-art methods.

==> Section_Tex_Files/back.tex <==
\ignore{\subsection{Algorithmic Fairness}
\label{related_work:Algorithmic_Fairness}

Fairness is defined as the ``absence of any prejudice or favoritism toward an individual or a group based on their inherent or acquired characteristics" \cite{mehrabi2019survey}. Conversely bias is ``a tendency, inclination, or prejudice toward or against something or someone" \cite{bias_psychologytoday_definition}. However, defining these concepts using mathematical notation such that they could be enforced on machine learning models is not as simply achieved. As a result, many have introduced different definitions and metrics that could capture the meaning of these concepts. Overall, definitions of fairness are often categorized under (a) group or (b) individual fairness definitions. Group fairness measures compare the performance of the model on some pre-defined groups, while individual fairness metrics consider the outcome for each individual, attempting to ensure that similar individuals are treated similarly \cite{caton2020fairness}. While these definitions are not fundamentally conflicting \cite{binns2020apparent}, their technical abstractions could make them so \cite{miconi2017impossibility, kleinberg2016inherent}.

In this section we will discuss the metrics used in this study, namely (i) statistical parity \cite{dwork2012fairness}, (ii) conditional statistical parity \cite{corbett2017algorithmic}, and (iii) equal opportunity \cite{hardt2016equality}. Mathematical definitions for all three metrics (i, ii, iii) were provided in Section \ref{section:background:ml_and_fairness}, here we will discuss the benefits and shortcomings of each one. All three measures, capture non-causal group level fairness of a system. We point the reader to \cite{narayanan2018translation, verma2018fairness, makhlouf2021machine, mehrabi2019survey, tashfia2021through, mitchell2021algorithmic} for a more complete list and discussion on each definition. Moreover, it is work noting that in recent years methods for choosing fairness and performance metrics to the task at hand have been proposed, such that the metric best reflects existing implicit preferences \cite{hiranandani2020fair}.

(i) Statistical parity is satisfied if both privileged and unprivileged groups have the same likelihood of being assigned to the positive class. This definition is attractive because it is simple to verify and requires no additional information or assumptions about the data \cite{chouldechova2020snapshot}. While this is one of the most simple definitions of fairness, it has been shown to most closely match people's idea of fairness \cite{srivastava2019mathematical} (The study specifically evaluated human perception in criminality and skin cancer risk prediction tasks). Additionally, this definition  can be useful when the labels are flawed or untrustworthy \cite{makhlouf2021machine}. There are also moral justifications for enforcing this metric discussed in \cite{hertweck2021moral}. However, there are many reported limitations to this definition as well. For one, it does not consider the possibility of a correlation between the label and sensitive attribute, thus in cases with unequal base rate, satisfaction of statistical parity can be misleading \cite{makhlouf2021machine}. Secondly, the problem of masking \cite{barocas2016big}, which is laziness or gaming of the system to accept individuals of the minority group randomly or according to different criteria \cite{makhlouf2021machine}, can occur when only attempting to satisfy this criteria. \cite{dwork2012fairness} discuss a number of scenarios where statistical parity can fail in making guarantees. 

(ii) Conditional statistical parity extends the definition of statistical parity by allowing a set of legitimate attributes to influence the outcome \cite{kamiran2013quantifying}. This measure allows for differences in decisions if they are explainable (for instance differences in qualifications in job hiring applications) \cite{makhlouf2021machine}, which was not possible in statistical parity. However, if the admissible variables are inappropriately selected, they could they could be used to game the system \cite{makhlouf2021machine}. 

(iii) Equal opportunity is satisfied if both privileged and unprivileged groups have equal true positive rates. Thus, this measure is not suitable if differing true negative rate can have significant fairness implications. 

Once metrics for the measurement of fairness were developed, many started looking into how it could be enforced. In other words, how bias, which would be defined as the level of deviation from the proposed metric, could be mitigated. The methods introduced for the task broadly fall into one of the following groups:

(a) pre-processing methods ``attack the problem by removing the underlying discrimination from the data before any modeling" \cite{d2017conscientious}. These methods often attempt to achieve fairness by relabeling examples \cite{nguyen2021fairness}, reweighting or resampling them \cite{romano2020achieving, li2019repair, kamiran2012data}, or feature transformations \cite{grgic2018beyond}. However, some have shown that certain data transformers can cause unfairness further down the ML pipeline \cite{biswas2021fair}. 

(b) in-processing methods try to modify the learning algorithms in order to remove discrimination during the model training process \cite{mehrabi2019survey}. Our bias mitigation algorithm falls into a sub-category of in-processing algorithms that enforce fairness using a regularization term \cite{konstantinov2021fairness, di2020counterfactual, bechavod2017learning, kamishima2012fairness}. While these methods have been shown to be effective, studies have noted that because these added constraints are non-convex, satisfying them could be difficult \cite{zafar2017fairnessbeyond}. \cite{zafar2017fairnessbeyond} also discuss how the performance of the classifier will depend on the dimension of the fair representation which can not be selected deterministically. 

(c) post-processing methods modify the results of a previously trained classifier to achieve the desired results on different groups \cite{friedler2019comparative}. These approaches often work by changing the labels in accordance to some fairness definition \cite{kamiran2012decision, pleiss2017fairness} or deriving a new predictor based on the outputs such that fairness is satisfied \cite{hardt2016equality}. Post-processing methods are specially useful for scenarios where the ML model is a black box and changes to the input or training can not be made \cite{mehrabi2019survey}. 

In recent years many have started looking into creating fair models using principles of causality \cite{rahmattalabi2022promises, loftus2018causal}. This is motivated by (a) the compatibility of causality with legal frameworks, (b) their robustness to spurious correlations \cite{simon1954spurious}, as well as (c) their interpretability for humans. One of the first places causality influenced fairness was in the definitions and notions of fairness \cite{kusner2017counterfactual, pearl2009causality, kilbertus2017avoiding}. As previously mentioned, statistical notions of fairness are often conflicting. Causal notions however, attempt to address this issue by looking at causation instead of correlation and solving the true source of the bias \cite{rahmattalabi2022promises}. Methods for capturing fairness violations and correcting for them using causal DAGs have been proposed in the literature \cite{yan2020silva, salimi2019interventional,pradhan2021interpretable, galhotra2022causal}. 

While we do not make use of causal notions of fairness, our methods fall in the intersection of fairness and causality as we utilize the causal generative process behind the data and modify the optimization process of the model according to the causal relationships between the features and the selection criteria. 

We end this section by pointing to two studies that bring into attention two topics that are sometimes overlooked in the fairness literature: (a) viability of datasets for the task and (b) stability of deep learning models in reported results. Since research into fairness of machine learning systems hinge on the datasets that are available, \cite{fabris2022algorithmic} perform a survey of 200 datasets employed in this field and provide documentation for them. They also perform in-depth analysis on the 3 most popular datasets in the field, discussing their limitations and possible alternatives. \cite{qian2021my}: discusses the current evaluation and testing procedures in the fairness literature for deep learning models. The paper argues that not getting results across multiple identical runs (something that is only done in 34\% of the fairness literature) makes results unreliable as deep learning systems have been shown to produce different results across multiple runs even when the structure or seeds don't change. This nondeterministic behavior (when even the seed is fixed) is caused by software implementations. As a result, they look into fairness variances caused by software implementations and find up to 12.6\% variance in fairness metrics across identical runs.

\subsection{Selection Bias}
\label{related_work:Selection_bias}
}
%However, we acknowledge that approaches for dealing with those case \cite{efron1994missing, van2018flexible} and the performance and fairness of those approaches \cite{zhang2021fairness, lakkaraju2017selective} have been studied. 


%Our research is related to algorithmic fairness and ML in the presence of selection bias. 



%In this section we will provide a brief overview of the related work. We will begin by looking into the fairness literature, discussing how fairness can be measured and mitigated (Section \ref{related_work:Algorithmic_Fairness}). Next we discuss viewing fairness from a statistical and causal perspective and the benefits and challenges of looking at the problem from these views (Section \ref{related_work:Algorithmic_Fairness}). We then examine related work on selection bias, beginning with basic understanding and the causal perspective of selection bias, and then moving on to how selection bias could effect fairness and what has already been done in this space (Section \ref{related_work:Selection_bias}). Finally we end this section by reviewing other studies that have bounded bias due to selection (Section \ref{related_work:Selection_bias:bounding}). 


\ignore{

Selection bias and its effects on fairness has received some attention in the fairness literature \cite{goel2020importance, du2021robust, wang2021analyzing, blum2019recovering, meyer2021certifying}. The study most closely related to ours is \cite{goel2020importance}. They authors of \cite{goel2020importance} also look at the problem from a causal perspective and discuss how data missingness, if ignored, could nullify the fairness guarantees that are given based on the training data. They look into different mechanisms corresponding to real-world scenarios where selection bias occurs, and discuss if the probability distributions needed for different fairness metrics would be recoverable in those scenarios. The missingness they focus on are cases where entire rows of data are missing (which is consistent with selection bias). Similar to our study they use causal inference to model this phenomenon. Selection is modeled as a node that is a child of it's deciding factor (which are a subset of the \textit{unobserved} set of variables), this node is then one of the parents of the observed versions of these nodes. The main differences between our study and \cite{goel2020importance} are: (1) \cite{goel2020importance} do not look into cases where selection bias is the cause of unfairness, in other words when the underlying data generative process is fair. As a result the structures presented in \cite{goel2020importance} are not comparable to the conditions given in Section \ref{section:introducing_bias_out_of_the_blue}. (2) They do not present bounds for the true fairness metrics and only discuss the possibility of full recoverability of the values. (3) They do not present a fair learning method in cases where the metric is not recoverable.  



Selection bias occurs when a random sample of a population of interest is not observed \cite{winship1992models}. This means that samples that are representative of certain sections of the population are missing. This missingness of data can be (i) completely at random (MCAR), (ii) at random (MAR), or (iii) not at random (MNAR). MCAR refers to cases where ``missingness does not depend on the values of variables in the data set subject to analysis" \cite{little1988test}. MAR on the other hand is when ``missingness does not depend on the missing values but may depend on observed values in the data set" \cite{little1988test}. Dealing with data missingness is often more easily done if MCAR assumption can be made \cite{potthoff2006can}. MNAR occurs when ``missingness depends not only on the observed data but also on the unobserved (missing) values" \cite{fielding2008simple}. It is important to note that the instances of data missingness we investigate in this study are when entire rows of data are missing, and not cases where labels or specific features are missing. 

As mentioned in Section \ref{section:introduction}, selection bias can occur in a vast variety of circumstances and datasets. As a result many have looked into methods for recovering from selection bias. Reweighting is one of the most commonly used approaches for dealing with selection bias. Reweighting methods modify the cost of an error on each training point according to some computed weights. These weights are often computed by estimation techniques using an unbiased sample of the population \cite{cortes2008sample}. Studies however, have shown that these estimations can have errors that can severely influence the performance of the model in downstream tasks \cite{cortes2008sample, liu2014robust}. As a result methods for calculating robust estimates/weights have been studied \cite{liu2014robust, huang2006correcting}. Modeling of selection bias using causal diagrams as another method for mitigation the bias has also been explored \cite{bareinboim2012controlling}. 
}
